Polyjuice: High-Performance Transactions via Learned Concurrency Control

Concurrency control algorithms are key determinants of the performance of in-memory databases. Existing algorithms are designed to work well for certain workloads. For example, optimistic concurrency control (OCC) is better than two-phase-locking (2PL) under low contention, while the converse is true under high contention. To adapt to different workloads, prior works mix or switch between a few known algorithms using manual insights or simple heuristics. We propose a learning-based framework that instead explicitly optimizes concurrency control via offline training to maximize performance. Instead of choosing among a small number of known algorithms, our approach searches in a "policy space" of fine-grained actions, resulting in novel algorithms that can outperform existing algorithms by specializing to a given workload. We build Polyjuice based on our learning framework and evaluate it against several existing algorithms. Under different configurations of TPC-C and TPC-E, Polyjuice can achieve throughput numbers higher than the best of existing algorithms by 15% to 56%.

==> Makefile <==
#DOC_NAME    := castm
DOC_NAME    := chamcc-paper

PS2PDF      := ps2pdf14

#use the following options to avoid the embedded font problem.
DVIPS       := dvips -j0 -Ppdf -Pdownload35 -G0 -t letter -D 1200 -Z -mode ljfzzz
LATEX       := pdflatex
FIG2DEV     := fig2dev

#use the following options to generate into a single html.
LATEX2HTML  := latex2html -split 0 -split +0 -link 0 -no_navigation -no_footnode -show_section_numbers -local_icons
DOXYGEN     := doxygen
BIBTEX	    := bibtex

BASE := Makefile $(wildcard *.tex) $(wildcard *.bib)
BASE := $(BASE) $(wildcard ./pic/*.eps)

PSOPT 	:=  -dNOPAUSE -dBATCH \
	-sDEVICE=pdfwrite -dPDFSETTINGS=/prepress\
	-dCompatibilityLevel=1.5 \
	-dCompressPages=true -dUseFlateCompression=false \
	-sPAPERSIZE=letter \
	-dSubsetFonts=true -dEmbedAllFonts=true \
	-dProcessColorModel=/DeviceGray \
	-dDetectBlends=true -dOptimize=true \
	-dDownsampleColorImages=true -dColorImageResolution=1200 \
	-dColorImageDownsampleType=/Average -dColorImageFilter=/FlateEncode \
	-dAutoFilterColorImages=false -dAntiAliasColorImages=false \
	-dColorImageDownsampleThreshold=1.50000 \
	-dDownsampleGrayImages=true -dGrayImageResolution=1200 \
	-dGrayImageDownsampleType=/Average -dGrayImageFilter=/FlateEncode \
	-dAutoFilterGrayImages=false -dAntiAliasGrayImages=false \
	-dGrayImageDownsampleThreshold=1.50000 \
	-dDownsampleMonoImages=true -dMonoImageResolution=1200 \
	-dMonoImageDownsampleType=/Average -dMonoImageFilter=/FlateEncode \
	-dAutoFilterMonoImages=false -dAntiAliasMonoImages=false \
	-dMonoImageDownsampleThreshold=1.50000

all: pdf


pdf: $(DOC_NAME).pdf

%.pdf: %.ps
	$(PS2PDF) $(PSOPT) $< $@
	@cat $(DOC_NAME).log | grep Warning

%.ps: %.dvi
	$(DVIPS) $< -o $@

%.dvi: $(BASE)
	@make clean
	set -x
	$(LATEX) $*.tex
	$(BIBTEX) $*
	$(LATEX) $*.tex
	$(BIBTEX) $*
	$(LATEX) $*.tex

plot:
	@cd gnuplot/scripts; ./plot_all.sh

html: $(DOC_NAME)/$(DOC_NAME).html

%.html: $(BASE)
	@rm -rf $(DOC_NAME)
	$(LATEX2HTML) $*.tex

clean:
	@rm -rf *.pdf *.ps *.dvi *.aux *.log *.bbl  *.blg *.idx *.out *~ pic/*~ $(DOC_NAME)

.PHONY: clean all pdf html

### Makefile ends here


==> optimization.tex <==
\section{Optimization}
\label{sec:optimization}

\subsection{Training configuration}
\label{subsec:train-conf}
There is no denying that concurrency control is crucial in database systems.
However, database performance is not decided only by concurrency control.
Some configurations of database also make key contribution to the overall system performance.
On the other hand, some of these key configurations rely on human knowledge and manual tunning, 
making it hard to find the optimal settings.
Therefore, {\sys} can take some of configurations into training set as an optimization, using training moudule to 
generate a learned settings of configurations.
In our implementation, only one configuration is taken, which is the "transaction buffer size", 
deciding how many latest finished transactions' metadata will be kept.
Cache locality is worse with small "transaction buffer size" value, and there are false-aborts with big value.
To confirm the influence caused by cache locality, 
we compare TPC-C mix workload with a large buffer size (32) to one with the learned buffer size (9). 
The result shows that the former one's cache miss rate is 8.46\% while the latter one's is 12.43\%.
The reason why we just take one configuration is that we do not want to make the exploration space too huge for training module.
And "transaction buffer size" can make a noticeable throughput difference to TPC-C workload.

\subsection{Lock implementation}
\label{subsec:train-conf}
Mix locking implementation, mcslock and spinlock.
